Switching Categoricity Behavior with a Given Degree

Given a noncomputable, computably enumerable set $D$, we construct a computable structure $G$ such that any two computable copies of $G$ are computably isomorphic while there are two $D$-computable copies of $G$ that are not $D$-computably isomorphic. In other words, $G$ is computably categorical, but not computably categorical relative to $D$. Conversely, we construct a computable structure that is not computably categorical, but is computably categorical relative to $D$. These results differ from those in the literature regarding computable categoricity and its relativiziations because the degree $D$ is given instead of constructed. Our work negatively answers a question of Downey, Harrison-Trainor and Melnikov in the computably enumerable case.

==> Other_Notes.tex <==
\iffalse

\section{To be Deleted}

\subsection{The formal framework for 1-true stages and $\sigma$-injuries}

\begin{definition} Global 1-true stages.

A global 1-true stage ordering is a computable partial ordering $\preccurlyeq$ on $\mathbb{N}^{<\mathbb{N}}$ that satisfies the following properties:

\begin{enumerate}
    \item $\langle \rangle \preccurlyeq \tau$ for all $\tau$;

    \item If $\sigma\preccurlyeq\tau$, then $\sigma\subseteq\tau$;

    \item For each $X\in \mathbb{N}^{\mathbb{N}}$, there is an infinite sequence of initial segments of $X$ such that $\tau_0 \preccurlyeq \tau_1 \preccurlyeq... \subset X$; and

    \item For every $\tau\subset \sigma \subset \rho$, if $\tau \preccurlyeq \rho$, then $\tau\preccurlyeq \sigma$.
\end{enumerate}

\end{definition}

When $\sigma \preccurlyeq \tau$, we say that $\tau$ believes $\sigma$. For substrings defined as in property (2), we say that $\tau$ is $X$-true and write $\tau \preccurlyeq X$.

\begin{definition}
    We say that $\preccurlyeq$ is complete if, for every $X\in\mathbb{N}^{\mathbb{N}}$ we have that $\mathcal{T}_X:=\langle \tau \in \mathbb{N}^{<\mathbb{N}}: \tau \preccurlyeq X\rangle\equiv_T X'$ uniformly in $X$.
\end{definition}

\begin{theorem} [Montalbán]
    There is a complete, global, 1-true stage system.
\end{theorem}

Following Lachlan's notion of \textit{true stages}, our constructions will use $\mathcal{T}_\emptyset$ as their $\emptyset'$-oracle. As we cannot directly access $\mathcal{T}_\emptyset$, we will define a series of stages $\mathcal{T}_\sigma$ that approximate it in a computable way.

\begin{definition} $\sigma$ stages.

Consider an approximation of $\emptyset'$ via finite binary sequences $\sigma_s=\langle \sigma_{i\leq s,s} \rangle \in \mathbb{N}^{<\mathbb{N}}$ defined as follows:

\begin{enumerate}
    \item $\sigma_{0,0}=0$, and
    \item $\sigma_{i,s}= \begin{cases} 
      1 & \phi_i(i)\downarrow \text{ in $s$ steps} \\
      0 & \text{ Otherwise }
   \end{cases}.$
\end{enumerate}

Then, at stage $s$ we call $\mathcal{T}_{\sigma}=\langle \tau\in\mathbb{N}^{<\mathbb{N}}: \tau \preccurlyeq  \sigma_s \rangle$ the \textit{current} approximation of $\emptyset'$.
\end{definition}


\begin{figure}{Figure 1: Relations between different types of stages}
\centering
\includegraphics[width=12cm]{Images/TrustRelations.png}
\end{figure}

\begin{definition} Belief (?)

We say that our construction $\mathcal{T}_{\sigma_j}$-believes $\mathcal{T}_{\sigma_k}$ when  $\mathcal{T}_{\sigma_k}\subseteq\mathcal{T}_{\sigma_j}$ and $\tau\preccurlyeq {\sigma_j}$ for every $\tau \preccurlyeq {\sigma_k}$.
\end{definition}

As only $\emptyset$-true stages will be correct, we must consider injuries arising from the use of incomplete oracles in our construction.

\begin{definition}
$\sigma$-injuries.

Let $k<s$ and $|\mathcal{T}_{\sigma_k}|=l$. At stage $s$, if it is found that $\mathcal{T}_{\sigma_k}\neq \mathcal{T}_{\sigma_s}\upharpoonright_l$ we say that every strategy that has used oracle $\mathcal{T}_{\sigma_k}$ \textit{in order to carry out an action} has been $\sigma$-injured and requires attention. \todo{Can all injuries be consolidated?}
\end{definition}

As long as our constructions are able to successfully recover from $\sigma$-injuries, they will be able to properly carry out their work over the infinite path of $\emptyset$-true stages. In order to achieve this, they will follow these rules:

\begin{enumerate}
    \item They will always act with the current $\mathcal{T}_\sigma$ as an oracle;

    \item At the beginning of every stage, the current $\mathcal{T}_\sigma$ will be used to revisit, in order of priority, all previously initiated strategies in order to identify possible $\sigma$-injuries. In other words, they will update their set of $\mathcal{T}_\sigma$-beliefs at the beginning of every stage; and

    \item $\sigma$-injuries will take priority over regular injuries that arise from the interaction between strategies.
\end{enumerate}

We can observe that the relation between our stages respects the global poset relation.

\begin{lemma}
Let the relations between $\mathcal{T}_{\sigma_0}$, $\mathcal{T}_{\sigma_j}$, $\mathcal{T}_{\sigma_k}$, $\mathcal{T}_{\sigma_s}$, and $\mathcal{T_{\emptyset}}$ hold as expressed in figure 1. Then, the following two statements hold:

\begin{itemize}
    \item If our construction $\mathcal{T}_\emptyset$-believes $\mathcal{T}_{\sigma_s}$ and $\mathcal{T}_{\sigma_s}$-believes $\mathcal{T}_{\sigma_j}$, then it $\mathcal{T}_\emptyset$-believes $\mathcal{T}_{\sigma_j}$; and

    \item If our construction $\mathcal{T}_\emptyset$-believes $\mathcal{T}_{\sigma_s}$ but does not $\mathcal{T}_{\sigma_s}$-believe $\mathcal{T}_{\sigma_k}$, then it does not $\mathcal{T}_\emptyset$-believe $\mathcal{T}_{\sigma_k}$ either.
\end{itemize}




\end{lemma}




\subsection{An example}

Let us start by reworking the proof of the following corollary [follows from the main proof in "Relativizing Computable Categoricity"].

\begin{definition} Lowness.

    Let \textbf{d} be a c.e. degree. We say that \textbf{d} is low if and only if whenever $\Phi^\textbf{d}_e(e)\downarrow$, there is an $s$ such that $\Phi^{\textbf{d}[s]}_e(e)\downarrow$ with use $u$ and $\textbf{d}[s]\upharpoonright_u = \textbf{d}[t]\upharpoonright_u$ for all $t\geq s$. In other words, $\textbf{d}'\leq_T\emptyset'$.
\end{definition}

\begin{theorem}
There is a computable structure $\mathcal{A}$ and a low c.e. degree \textbf{c} such that $A$ is computable categorical but \textbf{not} computably categorical relative to \textbf{c}.
\end{theorem}

\begin{definition}[Requirements]

With index $i$ in $\mathbb{N}$, these are the main requirements we seek to satisfy.

\begin{itemize}

    \item  $L_i$: \textbf{c} is low;

    \item $R_i$: $\Phi_i^{\textbf{c}}:\mathcal{A}\to\mathcal{B}_i$ is not an isomorphism. With $\mathcal{B}_i=\Psi^{\textbf{c}}_i$ a $\textbf{c}$-computable copy of $\mathcal{A}$; and
    \item $S_i$: If $M_i\cong \mathcal{A}$, then $M_i$ is computably isomorphic to $\mathcal{A}$.
    
\end{itemize}

\end{definition}

\begin{proof}
    Proof via true stages.

    
{$L_i$-strategies}:
\begin{enumerate}
    \item Let $\textbf{c}$ be the empty set. Upon initialization at stage $s>1$, $\mathcal{T}_{\sigma}$ is used to check if $\Phi_s^{\textbf{c}[s]}(s)$ halts. If so, a restrain is put on \textbf{c} with the use of that computation, $u_s$.

    \item If revisited at stage $k$, $\mathcal{T}_{\sigma}$ is used to check if $\Phi_s^{\textbf{c}[k]}(s)$ halts. If so, a restrain is put on \textbf{c} with the use of that computation, $u_k$.

\end{enumerate}

{$R_i$-strategies}:

\begin{enumerate}
    \item Upon initialization at stage $i$, a large $n$ is chosen and the following components are created in $\mathcal{A}[i]$ and $\mathcal{B}[i]$:

   \begin{align*}
        a_{1} : 2, 5n+1 & \ \ \ \ b_{1} : 2, 5n+1 \\
        a_{2} : 2, 5n+2 & \ \ \ \ b_{2} : 2, 5n+2.
    \end{align*}

    \item Upon being revisited at stage $s$, $\mathcal{T}_{\sigma}$ is used to check if all currently active, higher priority $S$-strategies have enough information to determine if their mappings can be extended. Once this has been confirmed for all such strategies, $\mathcal{T}_{\sigma}$ is used to check if $\Phi_i^{\textbf{c}[s]}$ maps $a_{1}$ to $b_{1}$ and $a_{2}$ to $b_{2}$. 

    If the map is found with use $u$, the following loops are added to $\mathcal{A}$ and $\mathcal{B}$. If $L_i$ has been completed, underlined loops will be created with use $v>\max\{u,u_i\}$. Otherwise, we bound over the largest $\max\{u,u_j\}$ currently available.
    
    \begin{align*}
        a_{1} : 2, 5n+1, 5+3 & \ \ \ \ b_{1} : 2, 5n+1, \underline{5n+3} \\
        a_{2} : 2, 5n+2, 5+4 & \ \ \ \ b_{2} : 2, 5n+2, \underline{5n+4}.
    \end{align*}

    Similarly to before, $\mathcal{T}_{\sigma}$ is used to ensure all currently active, higher priority $S$-strategies have enough information. If so, we proceed with our diagonalization by enumerating the highest possible number to the left of $v$ we can. Our final configuration being as follows:

     \begin{align*}
        a_{1} : 2, 5n+1, 5+3 & \ \ \ \ b_{1} : 2, 5n+1, 5n+4 \\
        a_{2} : 2, 5n+2, 5+4 & \ \ \ \ b_{2} : 2,  5n+2, 5n+3.
    \end{align*}

\end{enumerate}

{$S_i$-strategies} follow the usual isomorphism pressing technique.
  
    Injuries arising from the interaction between strategies:

    \begin{itemize}
        \item As $L_i$ strategies only act by restraining initial segments of $R_i$, they cause no injuries to any other strategies.

        \item When enumerating an element $e$ into $\textbf{c}$, $R_i$ strategies will injure all $L_k$ strategies with $u_k>e$ alongside every $R_k$ that relied on $\textbf{c}\upharpoonright_e$. In order to recover from this, the construction must homogenize all affected components and restart their respective strategies.
    \end{itemize}

    $\sigma$-injuries:

   \begin{itemize}
 
       \item When $\sigma$-injured, $S_i$ strategies continue their work to extend their maps using the current $\mathcal{T}_\sigma$ as usual.
    
       \item When $\sigma$-injured, all affected $L_i$ strategies are restarted in order of priority along with their respective $R_i$'s.

       \item When $\sigma$-injured, $R_i$ strategies can act one of two ways. If no relevant $L_i$ and $S_i$ strategies are affected and $\Phi_i^{\textbf{c}[s]}$ behaves as expected, it continues as normal. Otherwise, it homogenizes it's elements and restarts.
   \end{itemize}

\todo{A more formal verification, and to see if more can be asked of $\mathcal{T}_\sigma$}

\end{proof}


\subsection{Proof 1: The first direction}

\begin{theorem}
    Given a noncomputable \textcolor{purple}{\st{low}} c.e. set $D$, there exists a computable directed graph $\mathcal{A}$ that is computably categorical but \textbf{not} computably categorical relative to $D$.
\end{theorem}

\textcolor{purple}{From Jere: \textbf{Considering that it seems we have both directions without using true stages I will delete this section later. I'll keep for a bit so that I can copy some of the notes. I will work on another third section at the end to work some ideas on the alternation.}}


\begin{definition}[Requirements]

For $e,i\in\NN$, we list our requirements that we seek to satisfy.

\begin{itemize}

    \item $R_e$: $\Phi_i^{D}:\mathcal{A}\to\mathcal{B}_i$ is not an isomorphism; and
    \item $S_i$: If $M_i\cong \mathcal{A}$, then $M_i$ is computably isomorphic to $\mathcal{A}$.
    
\end{itemize}

Here, $\mathcal{B}$ is a $D$-computable copy of $\mathcal{A}$ that we build alongside the latter.
\end{definition}

\begin{proof}

\textbf{$R_e$-strategies}:

\textcolor{purple}{Let $D$ be our noncomputable c.e.\ set. Let $d_s$ denote the last number enumerated into $D$ at the beginning of stage $s$, i.e. we define $d_s=x$ where $x\in D[s]$ but for all $t<s$, $x\not\in D[t]$, if such an $x$ exists. If no such $x$ exists, then let $d_s=d_{s-1}$. We now discuss the $R_e$-strategy.}

\textcolor{purple}{\textbf{Step 1:} Upon initialization at a stage $s$, a large $n^e_0$ is chosen. For this description, we let $n=n^e_0$. The following components are created in $\mathcal{A}[s]$ and $\mathcal{B}[s]$ (Underlined loops are erased in the next stage):}
        \begin{align*}
        a_{2n} : 2, 5n+1, 5n+2, \textcolor{red}{5n+3} & \ \ \ \ a_{2n+1} : 2, 5n+1, 5n+2, \textcolor{blue}{5n+4} \\
        \textcolor{darkgray}{b_{2n}}: 2, 5n+1, 5n+2, \underline{\textcolor{red}{5n+3}} & \ \ \ \ \textcolor{darkgray}{b_{2n+1}} : 2, 5n+1,5n+2, \underline{\textcolor{blue}{5n+4}}.
    \end{align*}

\textcolor{purple}{\textbf{Step 2:} Upon being revisited at a stage $s'>s$, $R_e$ asks the following question:
    \begin{itemize}
        \item[(i)] Does $\Phi_e$ correctly map the $\mathcal{A}[s']$-components into $\mathcal{B}[s']$?
    \end{itemize}
    If the answer is yes, we erase the underlined loops in $\mathcal{B}[s']$ and recreate the original configuration (This time, underlined loops are created with $D$-use $v> \max\{ use(\Phi_e),d_{s'}\}$):}
 \begin{align*}
        a_{2n} : 2, 5n+1, 5n+2, \textcolor{red}{5n+3} & \ \ \ \ a_{2n+1} : 2, 5n+1, 5n+2, \textcolor{blue}{5n+4} \\
        \textcolor{darkgray}{b_{2n}}: 2, 5n+1, 5n+2, \underline{\textcolor{red}{5n+3}} & \ \ \ \ \textcolor{darkgray}{b_{2n+1}} : 2, 5n+1,5n+2, \underline{\textcolor{blue}{5n+4}}.
    \end{align*}
    
    \textcolor{purple}{Otherwise, we stay in \textbf{Step 2}.}

\textcolor{purple}{\textbf{Step 3:} We will suppress the stage notation from this point on unless otherwise needed. Every time a component reaches this stage for the first time, $R_e$ will create a new pair of components associated with $\Phi_e$ that will start at \textbf{Stage 1} and run in parallel to all previously existing ones. We have a couple of cases.}

\textcolor{purple}{\textbf{Case 3.1}: If a small enough $D$-enumeration allows us to diagonalize, we create the following configuration:}
 \begin{align*}
        a_{2n} : 2, 5n+1, 5n+2, \textcolor{red}{5n+3} & \ \ \ \ a_{2n+1} : 2, 5n+1, 5n+2, \textcolor{blue}{5n+4} \\
        \textcolor{darkgray}{b_{2n}}: 2, 5n+1, 5n+2, \textcolor{blue}{5n+4} & \ \ \ \ \textcolor{darkgray}{b_{2n+1}} : 2, 5n+1,5n+2,\textcolor{red}{5n+3}.
    \end{align*}

    \textcolor{purple}{$R_e$ then halts work for all of its other parameters defined so far and moves to \textbf{Stage 4}.}

\textcolor{purple}{\textbf{Case 3.2}: If a small enough $D$-enumeration erases $\Phi_e$'s map over our current pair of components, we add the missing loops to $\mathcal{B}[s']$ and cease working on these components indefinitely.}

\textcolor{purple}{\textbf{Case 3.3}: If $d_{s'}>use(\Phi_e)$ no action is taken for this component.}

\textcolor{purple}{\textbf{Step 4:} This stage exists only to check that $\Phi_e$'s map has not been erased. If this happens, the strategy resumes working with its other components. Otherwise, no action is taken.}

\bigbreak

\textbf{$S_i$-strategies}:

\textcolor{purple}{Should be able to work as expected, mapping elements as they appear.}

\end{proof}

\subsubsection{Verification}

\begin{lemma}
   \textcolor{purple}{If $\Phi_e$ is not an isomorphism, $R_e$ will either create finitely many components or infinitely many components that do not affect any $S_i$ strategy.}
\end{lemma}

\begin{proof}
  \textcolor{purple}{As $\Phi_e$ is not an isomorphism, it might eventually fail to show up or create an incorrect map. In this case, we will have that some components of $R_e$ will be at \textbf{Step 2} indefinitely and, by definition, no new components will be created by the strategy.}

  \textcolor{purple}{If $\Phi_e$ appears and disappears infinitely often over a single pair of components, $R_e$ will cease working on the pair after the first time $\Phi_e$ disappears. How the strategy behaves now does not affect neither it's requirement nor any $S_i$ strategy. As, once created, every new $\mathcal{A}$-components is not affected by any $D$-enumeration and is uniformly discernible from any other one, $S_i$ will be able to successfully map them.}
\end{proof}

\begin{lemma}
   \textcolor{purple}{If $\Phi_e$ is an isomorphism, at least one component created by $R_e$ will reach \textbf{Step 4}.}
\end{lemma}

\begin{proof}
  \textcolor{purple}{It breaks here! Isomorphisms could create infinitely many components and "make the construction give up" in all of them before settling in.}
  

\end{proof}

\fi

\break

\section{The Chain}

\textcolor{purple}{From Jere: When thinking of the chain, it became clear that the hardest part of merging the previous two theorems would be the verification. There will be a type of nested permission going on that will require tighter and tighter windows as the construction grows. $R$ strategies will need permission to diagonalize from all lower priority $S$ strategies AND will be susceptible to the disappearance of the isomorphism they are working against when a low enough enumeration happens in their oracle.}

\subsection{Part I}

\begin{theorem}
    Given two noncomputable c.e. sets $C$ and $D$ with $C\leq_T D$, there exists a computable directed graph $\mathcal{A}$ that is computably categorical relative to $D$ but is $\textbf{not}$ computably categorical relative to $C$.
\end{theorem}

\begin{definition}[Requirements]

For $e,i\in\NN$, we list our requirements that we seek to satisfy.

\begin{itemize}

    \item $S_i$: If $M_i^D\cong \mathcal{A}$, then $M_i^{D}$ is $D$-isomorphic to $\mathcal{A}$; and
    \item $R_e$: $\Phi^C_e:\mathcal{A}\to\mathcal{B}$ is not an isomorphism.

\end{itemize}

Here, $\mathcal{B}$ is a fixed $C$-computable copy of $\mathcal{A}$ that we build alongside the latter.

\end{definition}

This construction will follow a similar structure to that of the previous two theorems. In order to make the process work we will introduce a \textit{joint permission module} which will keep track of \textit{joint enumerations} of $C$ and $D$.

\textcolor{purple}{From Jere: I just wanted to try and make it more straightforward to see when enumerations \textit{work} and when they do not. Evidently there will be lots of cases with this approach. }

\begin{proof}

    \textbf{The joint permission module}:

    Let $C$ and $D$ be our noncomputable c.e. sets. We will define our joint enumeration $\{C\sqcup D\}[s]$ as follows:
    
\begin{enumerate}
    \item At stage 1, $\{C\sqcup D\}[1]$ equals $\max\{C[1],D[1]\}$ if both $C[1]$ and $D[1]$ have done the first enumeration of an element of their respective sets. Otherwise, $\{ C \sqcup D \}[1]$ does not have an output.

    \item Upon being revisited at stage $n$, if $\{ C \sqcup D\}[s]$ has not produced an output yet, the module will wait until the stage $k$ where both $D[s]$ and $C[s]$ have done the first enumeration of an element of their respective sets, say at stages $k$ and $k-1$. Then, $\{ C \sqcup D\}[k]$ will equal $\max\{C[k],D[k-1]\}$.

    \item Upon being revisited at stage $n$, if $\{ C \sqcup D\}[s]$ last enumerated an element at stage $j$ and it has enumerated a total of $m$ elements, the module will wait until the stage $k$ where both $D[s]$ and $C[s]$ have done the $m+1$-th enumeration of an element of their respective sets, say at stages $k$ and $j+1$. Then, $\{ C \sqcup D\}[k]$ will equal $\max\{C(k),D(j+1)\}$.
\end{enumerate}
    
    With this, let $d_s$ denote the last number enumerated into $\{ C \sqcup D\}[s]$ at the beginning of stage $s$.

    When $\{C\sqcup D\}[s]$ enumerates an element as in the success case of point (1), we say that we had a \textit{joint enumeration}. Otherwise, we refer to the enumeration as a $C$-enumeration or a $D$-enumeration depending on which function was the last one to enumerate the required element needed to properly define $\{C\sqcup D\}[s]$. 

    \bigbreak

    \textbf{$R_e-$strategies}:

    \textbf{Step 1:} Upon initialization at a stage $s$, a parameter $n^e_0$ is chosen to be larger than any parameter picked in the construction so far. For this description, we let $n=n^e_0$. The following components are then created in $\mathcal{A}[s]$ and in $\mathcal{B}[s]$:

            \begin{align*}
        a_{2n} : 2, \textcolor{red}{5n+1} & \ \ \ \ a_{5n+1} : 2, \textcolor{blue}{5n+2} \\
        \textcolor{darkgray}{b_{2n}} : 2,\textcolor{red}{5n+1} & \ \ \ \ \textcolor{darkgray}{b_{2n+1}} : 2, \textcolor{blue}{5n+2}.
    \end{align*}

    \textcolor{purple}{From Jere: Step 2 is essentially the same as in the previous proof, the strategy only has the extra condition that it only proceeds once it has some certainty that the map $\Phi_e^C[s']$ will not vanish.}
    
    \textbf{Step 2:} 
    In this step, the $m_i[s']$ parameters work as in theorem 2.1.
    
    Upon being revisited at a stage $s'>s$, $R_e$ asks the following questions:
    \begin{itemize}
        \item[(i)] Which indices $i$ have the property that $m_i[s']>n$?
        \item[(ii)] Does $\Phi^{C[s']}_e$ map the three $\mathcal{A}[s']$-components above correctly into $\mathcal{B}[s']$? If this is the case, is the use of this computation smaller than $d_s$?
    \end{itemize}
    If there exist such indices $i$ in (i), then let $u^i_n[s']$ denote the use of the map $f_i[s']$ on the aforementioned $\mathcal{A}[s']$-components. If the answer is yes to both questions in (ii), we proceed to \textbf{Step 3}. Otherwise, next time we revisit the strategy we will return to \textbf{Step 2} and ask the same question (ii) until the answer is to both questions is yes (if ever) before proceeding.

\bigbreak

   \textcolor{purple}{From Jere: Step 3 is where the myriad of cases appear. Here, we have to account for both the permission that $R$ needs to diagonalize and the permission that the $S$ strategy needs to delete it's map plus the relation between their oracles and possible enumerations in any of them.}

    \textbf{Step 3:} We will suppress the stage notation throughout this description unless otherwise needed. This step breaks off into the following cases.

       \textcolor{purple}{From Jere: Case 3.1 is an immediate diagonalization, but we still have to check in case the map we diagonalized against vanishes in the future. Here, we will end up having components with infinitely many loops for maps that keep appearing and vanishing.}

    \textbf{Case 3.1}: Suppose there is no $i$ such that $m_i[s']>n$. Then we add new cycles in $\mathcal{A}$ and in $\mathcal{B}$ to diagonalize against $\Phi^C_e$ with the following configuration:
    
    \begin{align*}
        a_{2n} : 2, \textcolor{red}{5n+1}, \textcolor{blue}{5n+2}, \textcolor{blue}{5n+3}& \ \ \ \ a_{2n+1} : 2, \textcolor{red}{5n+1}, \textcolor{blue}{5n+2}, \textcolor{red}{5n+4} \\
        \textcolor{darkgray}{b_{2n}} : 2, \textcolor{red}{5n+1}, \textcolor{blue}{5n+2}, \textcolor{red}{5n+4}& \ \ \ \ \textcolor{darkgray}{b_{2n+1}} : 2, \textcolor{red}{5n+1},\textcolor{blue}{5n+2},\textcolor{blue}{5n+3}.
    \end{align*}
    
    This component will be revisited at all further stages to check if the diagonalization still holds under new enumerations.

     \textbf{Subcase 3.1.1} \textcolor{purple}{(From Jere: Naming!)}:
    
    If a small enough \textit{joint enumeration} erases both the mapping of $\Phi_e^{C[s']}$ and makes it so $m_i[s']<n$ for every $i$ over the component, we will create the following configuration:

     \begin{align*}
        a_{2n} : 2, {5n+1}, {5n+2}, \textcolor{blue}{5n+3}& \ \ \ \ a_{2n+1} : 2, {5n+1}, {5n+2}, \textcolor{red}{5n+4} \\
        \textcolor{darkgray}{b_{2n}} : 2, {5n+1}, {5n+2}, \textcolor{blue}{5n+3}& \ \ \ \ \textcolor{darkgray}{b_{2n+1}} : 2, {5n+1},{5n+2},\textcolor{red}{5n+4}.
    \end{align*}

    The strategy will continue to work with the component as if in $\textbf{Step 2}$, only caring about the latest set of loops.
    
    \textbf{Subcase 3.1.2} \textcolor{purple}{(From Jere: Work in progress from here on)}:

     If a small enough $C$ enumeration makes it so $m_i[s']<n$ but the mapping of $\Phi_e^{C[s']}$ is preserved, we create the following configuration 

\begin{align*}
        a_{2n} : 2, \textcolor{red}{5n+1}, \textcolor{blue}{5n+2}, \textcolor{blue}{5n+3}, \textcolor{red}{5n+5} & \ \ \ \ a_{2n+1} : 2, \textcolor{red}{5n+1}, \textcolor{blue}{5n+2}, \textcolor{red}{5n+4},\textcolor{blue}{5n+6} \\
        \textcolor{darkgray}{b_{2n}} : 2, \textcolor{red}{5n+1}, \textcolor{blue}{5n+2}, \textcolor{blue}{5n+3}, \textcolor{blue}{5n+6}& \ \ \ \ \textcolor{darkgray}{b_{2n+1}} : 2, \textcolor{red}{5n+1},\textcolor{blue}{5n+2},\textcolor{red}{5n+4},\textcolor{red}{5n+5}.
    \end{align*}

    \textbf{Case 3.2}: Suppose there exist indices $i$ such that $m_i[s']>n$ and so the $D$-parameters $u^i_n$ are defined. Then, homogenize the components in $A_n$ in the following way:
        %\begin{align*}
        %a_{2n} : 2, 5n+1, 5n+2 & \ \ \ \ b_{2n} : 2, 5n+1, 5n+2 \\
        %a_{2n+1} : 2, 5n+1, 5n+2 & \ \ \ \ b_{2n+1} : 2, 5n+1, 5n+2,
    %\end{align*}
    \begin{align*}
        a_{2n} : 2, 5n+1, 5n+2 & \ \ \ \ a_{2n+1} : 2, 5n+1, 5n+2 \\
        \textcolor{darkgray}{b_{2n}} : 2, 5n+1, 5n+2 & \ \ \ \ \textcolor{darkgray}{b_{2n+1}} : 2, 5n+1, 5n+2,
    \end{align*}
    \begin{figure}[h]
   \centering
   \makebox[\textwidth][c]{\includegraphics[width=.8\textwidth]{Images/S3.png}}
    \caption{}
    \end{figure}
    
    \noindent and check if $d_{s'}<\min\{u^i_n : \text{$i$ is such that $m_i[s']>n$}\}$ (we refer to this property of $d_{s'}$ as $d_{s'}$ \textit{being small enough}). If $d_{s'}$ is small enough, then we add additional cycles to the components in $A_n$ to diagonalize against $\Phi_e$ as follows:
      %  \begin{align*}
        %a_{2n} : 2, 5n+1, 5n+2, 5n+3 & \ \ \ \ b_{2n} : 2, 5n+1, 5n+2, 5n+4 \\
        %a_{2n+1} : 2, 5n+1, 5n+2, 5n+4 & \ \ \ \ b_{2n+1} : 2, 5n+1, 5n+2, 5n+3.
    %\end{align*}
        \begin{align*}
        a_{2n} : 2, 5n+1, 5n+2, \textcolor{red}{5n+3} & \ \ \ \ a_{2n+1} : 2, 5n+1, 5n+2, \textcolor{blue}{5n+4} \\
        \textcolor{darkgray}{b_{2n}} : 2, 5n+1, 5n+2, \textcolor{blue}{5n+4} & \ \ \ \ \textcolor{darkgray}{b_{2n+1}} : 2, 5n+1, 5n+2, \textcolor{red}{5n+3}.
    \end{align*}
    
    After adding these new cycles, for all $S_i$-strategies where $i$ is such that $m_i[s']>n$, $R_e$ redefine $m_i[s'+1]=n$. $R_e$ does not need to take any further action. Otherwise, if $d_{s'}>u^i_n$ for some $i$, $R_e$ defines a new large $n^e_1$, and begins taking the previous steps with this parameter in mind, and lets the next strategy act.
    To be explicit, the strategy will create new components for this $n^e_1$ as in \textbf{Step 1} and subsequently try to add these components to the list of current active components as described in \textbf{Step 2} when the strategy is revisited.
    
\end{proof}

    
\subsection{Part II}


%\begin{figure}[h]
   % \centering
   % \makebox[\textwidth][c]{\includegraphics[width=1.4\textwidth]{Images/AB.png}}
   % \caption{View of the $\mathcal{A,B}$-components.}
%\end{figure}

%\break

%\begin{figure}[h]
   % \centering
   % \makebox[\textwidth][c]{\includegraphics[width=1.3\textwidth]{Images/FlowChart.png}}
  %  \caption{Flowchart of $R_e$.}
%\end{figure}




